Better Language Models of Code through Self-Improvement

Pre-trained language models for code (PLMCs) have gained attention in recent research. These models are pre-trained on large-scale datasets using multi-modal objectives. However, fine-tuning them requires extensive supervision and is limited by the size of the dataset provided. We aim to improve this issue by proposing a simple data augmentation framework. Our framework utilizes knowledge gained during the pre-training and fine-tuning stage to generate pseudo data, which is then used as training data for the next step. We incorporate this framework into the state-of-the-art language models, such as CodeT5, CodeBERT, and UnixCoder. The results show that our framework significantly improves PLMCs' performance in code-related sequence generation tasks, such as code summarization and code generation in the CodeXGLUE benchmark.

==> emnlp_archived/PL_NL.tex <==
\begin{table*} [t]
\begin{center}
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{p{12cm}p{7cm}}
\begin{minipage}{0.75\textwidth}
\resizebox{\textwidth}{!}{
\begin{tabular}{lc c lc c c c c cc}
\toprule
Models & Beam sizes & Methods & Ruby & JavaScript & Go & Python & Java & PHP & Overall \\
\midrule
    RoBERTa & 10 &\cite{DBLP:journals/corr/abs-1907-11692} & 11.17 & 11.90 & 17.72 & 18.14 & 16.47 & 24.02 & 16.57 \\
%\midrule
PLBART & 10 &\cite{ahmad-etal-2021-unified}& 14.11 & 15.56 & 18.91 & 19.30 & 18.45 & 23.58 & 18.32 \\
%\midrule
PolyglotCodeBERT & 10 &\cite{DBLP:journals/corr/abs-2112-02043} & 14.75 & 15.80 & 18.77 & 18.71 & 20.11 & 26.23 & 19.06 \\
%\midrule
UniXCoder & 10 &\cite{guo-etal-2022-unixcoder} & 14.87 & 15.85 & 19.07 & 19.13 & 20.31 & 26.54 & 19.30 \\
\midrule
CodeBERT & 1 & Baseline          & 12.04 & 14.73 & 17.58 & 18.47 & 17.62 & 23.44 & 17.31   \\
         %&   & Continue training & 12.04 & 15.47 & 17.63 & 18.55 & 17.85 & 23.60 & 17.52 \\
         &   & DistilCodeGen               & 12.40 & 15.44 & 18.52 & 19.09 & 18.31 & 24.46 & 18.04 \\
\cdashline{2-10}
         & 5 & Baseline          & 12.31 & 15.76 & 18.12 & 19.09 & 18.37 & 24.85 & 18.08 \\
         %&   & Continue training & 12.51 & 16.44 & 18.25 & 19.25 & 18.65 & 24.98 & 18.35 \\
         &   & DistilCodeGen               & 12.55 & 16.41 & 18.69 & 19.50 & 18.88 & 25.21 & 18.54 \\
\cdashline{2-10}
         & 10 & Baseline          & 12.22 & 15.78 & 18.01 & 19.09 & 18.42 & 25.06 & 18.10\\
         %&    & Continue training & 12.25 & 16.56 & 18.08 & 19.25 & 18.73 & 25.16 & 18.34 \\
         &    & DistilCodeGen               & 12.52 & 16.39 & 18.66 & 19.50 & 18.92 & 25.28 & 18.54 \\
\midrule
CodeT5 (base) & 1 & Baseline          & 14.80 & 15.57 & 19.57 & 19.86 & 19.87 & 25.33 & 19.17 \\
       %&   & Continue training & 15.01 & 15.59 & 19.40 & 19.61 & 19.88 & 25.18 & 19.11 \\
       &   & DistilCodeGen & 15.46 & 16.22 & 20.12 & 20.36 & 20.25 & 26.25 & 19.78 \\
       %&   & DistilCodeGen (multi-languages) & \textbf{15.45} & \textbf{16.22} & \textbf{20.06} & \textbf{20.34} & \textbf{20.35} & \textbf{26.16} & \textbf{19.76} \\
\cdashline{2-10}
       & 5 & Baseline          & 15.23 & 16.18 & 19.95 & 20.42 & 20.26 & 26.11 & 19.69 \\
       %&   & Continue training & 15.27 & 16.04 & 19.78 &  20.03 & 20.41 & 26.06 & 19.60 \\
       &   & DistilCodeGen & 15.60 & \textbf{16.51} & 20.26 & \textbf{20.59} & 20.44 & 26.46 & 19.97 \\
       %&   & DistilCodeGen (multi-languages) & \textbf{15.48} & \textbf{16.45} & \textbf{20.23} & \textbf{20.60} & \textbf{20.50} & \textbf{26.47} & \textbf{19.96} \\
\cdashline{2-10}
       & 10 & Baseline          & 15.29 & 16.18 & 19.95 & 20.42 & 20.26 & 26.10 & 19.70 \\
       %&    & Continue training & 15.39 & 15.92 & 19.81 & 20.11 & 20.41 & 26.07 & 19.61 \\
       &    & DistilCodeGen & \textbf{15.70} & 16.47 & \textbf{20.28} & 20.58 & \textbf{20.45} & \textbf{26.58} & \textbf{20.00} \\
       %&   & DistilCodeGen (multi-languages) & \textbf{15.45} & \textbf{16.52} & \textbf{20.24} & \textbf{20.58} & \textbf{20.47} & \textbf{26.44} & \textbf{19.95} \\
% \midrule % incorrect results
%     UniXCoder (base) & 1 & Baseline          & 14.83 & 15.39 & 18.95 & 18.66 & 19.37 & 24.99 & 18.70 \\
%        &   & DistilCodeGen & 15.35 & 15.46 & 19.40 & 19.04 & 19.93 & 25.71 & 19.15 \\
% \cdashline{2-10}
%        & 5 & Baseline          & 15.17 & 15.93 & 19.52 & 19.25 & 20.18 & 26.45 & 19.42 \\
%        &   & DistilCodeGen & 15.53 & 15.99 & 19.69 & 19.50 & 20.31 & 26.52 & 19.59 \\
% \cdashline{2-10}
%        & 10 & Baseline          & 14.74 & 15.84 & 19.31 & 19.12 & 20.11 & 26.75 & 19.31 \\
%        &    & DistilCodeGen & 15.53 & 15.89 & 19.67 & 19.51 & 20.30 & 26.55 & 19.58 \\
\midrule
    UniXCoder (base) & 1 & Baseline          & 14.83 & 15.39 & 18.95 & 18.66 & 19.37 & 24.99 & 18.70 \\
       &   & DistilCodeGen & 15.36 & 15.83 & 19.42 & 19.13 & 20.04 & 26.05 & \\ 
\cdashline{2-10}
       & 5 & Baseline          & 15.17 & 15.93 & 19.52 & 19.25 & 20.18 & 26.45 & 19.42 \\
       &   & DistilCodeGen & 15.37 & 19.95 & 19.73 & 19.55 & 20.45 & 26.69 & \\
\cdashline{2-10}
       & 10 & Baseline          & 14.74 & 15.84 & 19.31 & 19.12 & 20.11 & 26.75 & 19.31 \\
       &    & DistilCodeGen & 15.37 & 16.96 & 19.73 & 19.56 & 20.44 & 26.69 & \\

\bottomrule
\end{tabular}
}

\end{minipage}
\end{tabular}
}
\captionsetup{type=table}
\vspace{-0.5em}  
\caption{Results on code summarization task evaluated with smoothed BLUE-4. For CodeBERT and CodeT5, results with and without DistilCodeGen are reported from our experiments. Orther models' results are reported from each corresponding paper.
The ``Overall'' column presents average scores over six programming languages. Best resutls are in bold. 
%For CodeT5, we choose the already fine-tuned codet5-base-multi-sum checkpoint released on Hugging Face as Baseline, as well as initilization for Continue Training and DistilCodeGen models over 6 programming languages. 
%Each Baseline model of CodeBERT reported is fine-tuned from the available CodeBERT pretrained checkpoint individually for each language, and DistilCodeGen models are further tuned from these Baselines.
%Score for each PL in DistilCodeGen is averaged over three runs with different random seeds.
}\label{table:summarize}
\end{center}
\vspace{-1em}
\end{table*}


==> figures/plot_10.tex <==
\begin{figure}
%\centering
%\resizebox{\linewidth}{!}{
 \centerline{\includegraphics[width=1\linewidth]{media/plot_10.pdf}}
%}
\caption{
Scatter plot visualizing 
performance gap (in BLEU score) infered by different beam sizes (i.e 10 and 1) of $\theta_{fine-tuned}$
vs. 
performance gained (in BLEU score) by $\theta_{improved}$ infered with beam size of 10
}\label{figure:plot_10}
\vspace{-1em}
\end{figure}


==> figures/plot_5.tex <==
\begin{figure}
%\centering
%\resizebox{\linewidth}{!}{
 \centerline{\includegraphics[width=1\linewidth]{media/plot_5.pdf}}
%}
\caption{
Scatter plot visualizing 
performance gap (in BLEU score) infered by different beam sizes (i.e 10 and 1) of $\theta_{fine-tuned}$
vs. 
performance gained (in BLEU score) by $\theta_{improved}$ infered with beam size of 5
}\label{figure:plot_5}
\vspace{-1em}
\end{figure}


==> sections/exp-res_archived.tex <==
\section{Evaluation Results}

\input{tables/NL_PL}
\input{tables/PL_PL}

% In this section, we present the results of the proposed method. %applied on CodeT5 and CodeBERT for code summarization and code generation.
%The Baseline models are the released checkpoints for CodeT5, which are downstream task fine-tuned versions. However, we fine-tuned models task-specifically from a pre-trained checkpoint for CodeBERT by ourselves to obtain these Baseline.
% In summary, DistilCodeGen consistently outperform the Baseline models on every language and task in every single run. Our DistilCodeGen applied on CodeT5 achieve state-of-the-art results on code summarization in BLEU and on code generation on BLEU and CodeBLEU.
%It should be emphasized that with the presented method, each single run always outperforms the Baseline.
%However, for some languages, the margins seem to be small and running experiments on different random seeds is necessary to allow us to be more confident to claim that the method does work and gains performance.

% \subsection{Generative Tasks}

%\vspace{-0.5em}
\paragraph{Code Summarization}

Table~\ref{table:summarize} shows the performance of code summarization in term of smoothed BLEU-4
%We run beam search with three beam sizes as 1, 5, and 10 for each sub-task and model.
%All models after applying the method outperform their Baselines and Continue training versions across every programming language and beam size in every single experiment that we conducted.
Across all programming languages and beam sizes, all DistilCodeGen-applied models outperform their respective baselines.
Specifically, with CodeT5, the BLEU score is improved by +0.61, +0.28, and +0.31 for beams of sizes 1, 5, and 10 respectively.
+0.73, +0.46, and +0.44 are the improvement margins for CodeBERT.
These outcomes are also state-of-the-art across all programming languages for this assignment.
%By comparing with Continue training models, we observe that futher training the Baseline models degrade the overall performance for CodeT5, this is the sign of overfitting.
%In the case of CodeBERT, the Baseline models seem to be a bit under-trained, further training them on the train dataset gives a boost in performance, but still underperform Our models with the applied method.

\vspace{-0.5em}
\paragraph{Code Generation} 
%For this task, we employ CodeBLEU as our similarity function.
We show the results of this task for CodeT5 in Table~\ref{table:concode}.
%As in code summarization, we begin with the checkpoint released for code generation by CodeT5.
%However, we find that the checkpoint is severely under-trained, so we first make sure the Baseline is well-trained for this task.
%Indeed, further fine-tuning the released checkpoint gives a not marginal boost in performance for all three metrics as in Table~\ref{table:concode}.
%Then we choose this well-trained model as our Baseline.
With DistilCodeGen, performance gains are reported as follows: +0.5, +0.47, and +0.71 for CodeBLEU score, +0.75, +0.94, and +2.26 for BLEU score, +0.65, +1.30, and +0.25 for EM with beam size increasing from 1 to 10.
Together with code summarization, DistilGenCode helps achieve SOTA results on BLEU and CodeBLEU for code generation.
%The scores increase for all metrics, and for every beam size. The increase in CodeBLEU can be explained as we are optimizing directly on this metric, i.e we use it as our similarity function, and the increase in BLEU can be simply explained by that as optimizing CodeBLEU, we also partially optimize BLEU.

\vspace{-0.5em}
\paragraph{Code Translation} 
%For this task, we employ CodeBLEU as our similarity function.
We show the results of this task for CodeT5 in Table~\ref{table:translate}.

%\vspace{-0.5em}
% \subsection{Decoding Speed}
% An interesting observation that can be made when comparing performance across beam sizes is that by applying DistilCodeGen, inference with a beam of size 1 matches or even slightly outperforms the baselines using a beam of size 10 for the majority of programming languages in code summarization and for code generation in EM and BLEU score.
% Technically, for auto-regressive generative models, inference time complexity with beam search would be $O(B)$ with $B$ as the beam size.
% From this observation, with DistilCodeGen, we could achieve the same or even better performance in much less time only by reducing the beam size.
% This result is consistent with the observation of~\cite{kim-rush-2016-sequence}, which we believe to have a significant meaning in deploying deep learning models for real-world application, especially in code domains.
%This would make the deployment much faster and bring a better experience for the end users. The only cost to achieve this is the extra resource would be taken to generate pseudo dataset and continue fine-tuning the model with the proposed method.

%\input{tables/seq_prob}

%\vspace{-0.5em}
%\paragraph{Analysis.}
%%We observe that
%%There is a correlation between the beam size and the absolute improvement of the method % when looking at ...
%%This trend is also consistent for each sub-task (programming language).
%We hypothesize that what the method does is to reveal the sequence information generated by the model to itself, so that it can easily find the path to a more probable sequence in a sequential manner. At inference time, we aim to look for the sequence with the highest probability, but finding the mode of the whole sequence distribution is intractable, so we estimate it with beam search. First, the method forces the model to be better at selecting high probability sequences by picking the high probability token candidates at each position, from left to right. This results in the sequence distribution $p(\tvec \given \svec;\theta)$ to be more extreme or has a low entropy, concentrating probability mass to a small number of sequences.
%%This  makes the model easier to get the high probability sequences.
%Nevertheless, if the model is not sufficiently good enough, high probability does not guarantee a good candidate translation sequence. So, instead of generating candidate sequences that maximize probability only, we take the groundtruth into account and maximize the quantity $sim(\tvec \given \yvec) p(\tvec \given \svec)$. Now we are forcing the model to present the sequence probability distribution with low entropy with mass probability concentrated to a few probable sequences that are closer to the truths.


%We prove this statement quantitatively and qualitatively. 

%Why does our method increase the sequence prob? The following example analyzes the logic. At each step, the model try to shape the distribution q(token t | previous target tokens, source) so that the . It is like the model can look ahead to know which seq would result in high prob and try to shape the distribution q() so that q (token t = token t by beam search target | pre target tokens, source) be high, with beam search target is a seq prob. 

%First, in Table~\ref{table:seq_prob}, we compare the sequence probability of the sequences generated by model with greedy decoding. 

%Case 1: given the truth sequence, as comparison with the partial sequence prob, we see that our method makes the greedy decoding easier to search for to sequence Case 2: given what the hell is this???? 

%\vspace{-0.5em}
%\paragraph{Comparing to other methods bridging gap between training and inference}
%Since bridging the gap is one of the key ingredients in the method, we compare the complexity of our method to others.  
%
%Besides, in early experiments, we also try, sequence-level minimmu risk training as in te paper (), but we do not see much better improvement in performace compared to the method we are using, while the cost for running these method are significantly higher, including the following steps after we have the fine-tuning model: (step1, step2, step3). Our method with much lower resource required achive similar improvement. 
%
%We also consider the setup when we iteratively train with and creating the pseudo data in the following manner:
%1. at the beggining of each epoch, we use the current model to generate pseudo data from train data, then use this new pseudo data to train model for the current epoch
%2. at each step, we first generate pseudo data for the current batch, then perform forward pass on this new pseudo data batch, perform mini-batch gradient descent to update the parameters
%
%The cost is for these above frameworks is significantly large but the emperical result gains in performace is only slightly better. we hypothesize that it is be cause, the method only help the model make the seuqnec distribution more extreme .... So not much gains.

%\subsection{New training paradigm for generative auto-regressive models of code: Pre-training, Fine-tuning, Distilling}


==> sections/method_archived.tex <==
\section{Method}

\input{algorithms/method}
\input{tables/PL_NL}
\input{figures/method}

%However, strictly following this training procedure is difficult if the student network is trained from scratch. Since we are not optimizing the model directly on the ground truth training data, but predictions of the teacher, it would take a very long time for convergence or even diverge. In the paper~\cite{kim-rush-2016-sequence}, the authors also begin training from a fine-tuned model with a smaller learning rate.

We simplify the setting of sequence-level interpolation distillation by only considering the case when the student has the identical architecture and has parameters $\theta$ initialized the same as the teacher.
From our perspective, instead of viewing the method with this setting under the knowledge distillation framework, we interpret it as bridging the gap between training and inference procedure of generative models.

We start with a well-trained Seq2Seq model with parameters $\theta$ on a specific task. The $\theta$ is derived from training the model with the MLE objective
\begin{equation}\label{eq:1}
\mcL(\theta) =
    \sum_{j=1}^{J} \log p(t_j = y_j \given \svec, \yvec_{<j};\theta)
\end{equation}
%In training, the objective is to predict the distribution of the next token conditioned on the source sentence and the previous tokens from the truth target sequence. 
However, in inference, what the model actually does is to predict the distribution $p(t_j \given \svec, \tilde{\yvec}_{<j})$ of the next token given the source sentence and the previous tokens that is generated by itself, where $\tilde{\yvec}$ is a sequence generated by the model with a given source sentence.
%\begin{equation}\label{eq:3}
%\tilde{\yvec} = 
%\argmax_{\tvec \in \mcT} p(\tvec \given \svec)
%\end{equation}
%The $\argmax$ operation is usually approximated with beam search.
%and the model has never been trained to model these distributions. 
The $p(t_j \given \svec, \yvec_{<j})$ is different from $p(t_j \given \svec, \tilde{\yvec}_{<j})$ as suggested by ~\cite{DBLP:journals/corr/RanzatoCAZ15}.
%from training dataset, after fine-tuned on a specific task, 
This mismatching between training and inference results in the accumulative errors incrementally each time the model generates a new token and uses it as input to predict the next one in inference.

%Given well-trained models on tasks such as code summarization or code generation by pre-training and fine-tuning paradigm, we show that these models can further be fine-tuned to gain even higher performance with a simple fine-tuning procedure. The original work proposed a sequence knowledge distillation for NMT, the main type of model they applied their technique is Seq2Seq. 

%%Here we formulate the teacher as the well-trained network on the original train data, including the parameters and 
This observation indicates that the model should be exposed to its predicted sequences in training.
This can be done via replacing the $\yvec$ by $\tilde{\yvec}$ in Equation (\ref{eq:1})
%, which results in
%\begin{equation}\label{eq:4}
%\mcL(\theta) =
%    \sum_{j=1}^{J} \log p(t_j = y_j \given \svec, \tilde{\yvec}_{<j})
%\end{equation}
Then we continue training the model with this new objective.
Nevertheless, the problem emerges as the generated sequences are not perfectly correct and contain errors within each prediction.
%Training the model on such an erroneous dataset would lead to confirmation bias and can cause the parameters converge to the irrelevant solution, ultimately making the generalization even worse. 
%We also aims to have an ideal model that should be trained so that the higher the predicted sequence probability $p(t|s,\theta)$ the better the prediction should be or the closer to grourth truth. Because our model can never be perfect, so higher probabilities do not guarantee to be better. 
This leads to the motivation of integrating back the training data back to training.
%train our model on a dataset such that we can expose the model's predicted sequences to itself but still keep the original objective of generating correct sequences. 
From here, we follow the sequence-level interpolation distillation approach to achieve this purpose.
%We replace the equation (\ref{eq:3}) with
The predicted sequence is now generated as

\begin{equation}\label{eq:2}
\tilde{\yvec} = 
\argmax_{\tvec \in \mcT} sim(\tvec, \yvec) p(\tvec \given \svec)
\end{equation}
where $sim$ is a function measuring closeness.

Evaluating $sim(\tvec, \yvec) q(\tvec \given \svec)$ for every possible sequences is impossible, we can approximate the sequence by running beam search and choosing
\begin{equation}\label{eq:3}
\tilde{\yvec} \approx 
\argmax_{\tvec \in \mcT_K} sim(\tvec, \yvec)
\end{equation}
where $\mcT_K$ is the $K$-best list from beam search. 
In this paper, we take $sim$ to be smoothed sentence-level BLEU for code summarization and CodeBLEU for code generation.

%With the objective kept the same as (\ref{eq:4}), 
We fine-tune the model with these new generated target sequences in order to both capture the model behavior at generating sequences and keep the objective close to predicting the correct target sequences.


We refer this whole process of continuing fine-tuning a model on data generated by itself as DistilCodeGen in this paper.
In summary, given a well-trained generative language model on a specific task, DistilCodeGen exposes the model to its predictions by simply generating predictions for the train dataset by Equation~\ref{eq:3}. These predictions are combined with the original data by replacing the target ground truths to form the new dataset, which we call pseudo datasets within the scope of this paper. The final step is to continue fine-tuning the trained model on the pseudo dataset with the objective in Equation~\ref{eq:1} with $\yvec$ substituted by $\tilde{\yvec}$.

%%-------
%This observation indicates that the model should be expose to its predicted sequences in training. 
%
%The important part is how qualitative the new pseudo dataset is.
%
%On the order hand, 
%Notably, despite the above technique and analysis being mostly for sequence to sequence models, they are also true for other generative frameworks such as auto-regressive decoder-only. In such cases, the source sentence $\svec$ in $p(\tvec \given \svec;\theta)$ can be seen as an empty sentence.


==> tables/ablation_NL_PL.tex <==
\begin{table} [t]
\captionsetup{font=scriptsize}
%\begin{center}
\centering
\resizebox{\columnwidth}{!}{
%\begin{tabular}{p{12cm}p{7cm}}
%\begin{minipage}{0.75\textwidth}
%\resizebox{\textwidth}{!}{
\begin{tabular}{lc c c c c c}
\toprule
Models & Beam sizes & Methods & EM & BLEU & CodeBLEU \\ 
\midrule
    UniXCoder & & Baseline               & 21.50 & 38.28 & 40.85\\
       & 1 & From $\theta_{pre-trained}$ & 20.45 & 36.50 & 39. 09 \\
       &    & From $\theta_{fine-tuned}$ & \textbf{22.10} & \textbf{38.56} & \textbf{40.96} \\
\cdashline{2-6}
       & & Baseline                      & 22.05 & 37.53 & 40.11 \\
       & 5 & From $\theta_{pre-trained}$ & 21.70 & 34.50 & 37.64 \\
       &    & From $\theta_{fine-tuned}$ & \textbf{22.30} & \textbf{37.88} & \textbf{40.42} \\
\cdashline{2-6}
       &  & Baseline                      & 22.00 & 37.18 & 39.78 \\
       & 10 & From $\theta_{pre-trained}$ & 22.05 & 32.60 & 36.15 \\
       &    & From $\theta_{fine-tuned}$  & \textbf{22.30} & \textbf{37.49} & \textbf{40.05} \\
\bottomrule
\end{tabular}
}

%\end{minipage}
%\end{tabular}
%}
%\captionsetup{type=table}
\vspace{-0.5em}  
\caption{CodeT5 performance results on code generation evaluated with EM, BLEU, and CodeBLEU. For CodeT5, results with and without \methodname are reported from our experiments. Orther models' results are reported from each corresponding paper. Best results are in bold.
}\label{table:ablation_concode}
%\end{center}
\vspace{-1em}
\end{table}


==> tables/ablation_PL_NL.tex <==
\begin{table*} [t]
\begin{center}
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{p{12cm}p{7cm}}
\begin{minipage}{0.75\textwidth}
\resizebox{\textwidth}{!}{
\begin{tabular}{lc c lc c c c c cc}
\toprule
Models & Beam sizes & Methods & Ruby & JavaScript & Go & Python & Java & PHP & Overall \\
\midrule
    UniXCoder (base) & 1 & Baseline          & 14.83          & 15.39          & 18.95          & 18.66          & 19.37          & 24.99          & 18.70 \\
       &   & From $\theta_{pre-trained}$     & 15.35          & 15.46          & 19.40          & 19.04          & 19.93          & 25.71          & 19.15 \\
       &   & From $\theta_{fine-tuned}$      & \textbf{15.36} & \textbf{15.83} & \textbf{19.42} & \textbf{19.13} & \textbf{20.04} & \textbf{26.05} & \textbf{19.31} \\ 
\cdashline{2-10}
       &   & Baseline                   & 15.17          & 15.93          & 19.52          & 19.25          & 20.18          & 26.45          & 19.42 \\
       & 5  & From $\theta_{pre-trained}$& \textbf{15.53} & \textbf{15.99} & 19.69          & 19.50          & 20.31          & 26.52          & 19.59 \\
       &   & From $\theta_{fine-tuned}$ & 15.37          & 15.95          & \textbf{19.73} & \textbf{19.55} & \textbf{20.45} & \textbf{26.69} & \textbf{19.62} \\
\cdashline{2-10}
       &    & Baseline                   & 14.74          & 15.84          & 19.31          & 19.12          & 20.11          & \textbf{26.75} & 19.31 \\
       & 10 & From $\theta_{pre-trained}$& \textbf{15.53} & 15.89          & 19.67          & 19.51          & 20.30          & 26.55          & 19.58 \\
       &    & From $\theta_{fine-tuned}$ & 15.37          & \textbf{15.96} & \textbf{19.73} & \textbf{19.56} & \textbf{20.44} & 26.69          & \textbf{19.63} \\

\bottomrule
\end{tabular}
}

\end{minipage}
\end{tabular}
}
\captionsetup{type=table}
\vspace{-0.5em}  
\caption{Results on code summarization task evaluated with smoothed BLUE-4. For CodeBERT and CodeT5, results with and without \methodname are reported from our experiments. Orther models' results are reported from each corresponding paper.
The ``Overall'' column presents average scores over six programming languages. Best resutls are in bold. 
%For CodeT5, we choose the already fine-tuned codet5-base-multi-sum checkpoint released on Hugging Face as Baseline, as well as initilization for Continue Training and \methodname models over 6 programming languages. 
%Each Baseline model of CodeBERT reported is fine-tuned from the available CodeBERT pretrained checkpoint individually for each language, and \methodname models are further tuned from these Baselines.
%Score for each PL in \methodname is averaged over three runs with different random seeds.
}\label{table:ablation_codesum}
\end{center}
\vspace{-1em}
\end{table*}


==> tables/r1_r2.tex <==
% \begin{table} [t]
% \captionsetup{font=scriptsize}
% %\begin{center}
% \centering
% \resizebox{\linewidth}{!}{
%\begin{tabular}{p{12cm}p{7cm}}
%\begin{minipage}{0.75\textwidth}
%\resizebox{\textwidth}{!}{

\begin{table*} [t]
\begin{center}
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{p{12cm}p{7cm}}
\begin{minipage}{0.75\textwidth}
\resizebox{\textwidth}{!}{

\begin{tabular}{lc c c c c c c c     c c c c c c c c c c c c}
\toprule
\multirow{2}{*}{Metrics} & \multicolumn{6}{c}{UniXCoder} & \multicolumn{6}{c}{CodeBERT} & \multicolumn{6}{c}{CodeT5} \\ 
\cmidrule(lr){2-7}\cmidrule(lr){8-13}\cmidrule(lr){14-20}
& Ruby & Javascript & Go & Python & Java & PHP & Ruby & Javascript & Go & Python & Java & PHP & Ruby & Javascript & Go & Python & Java & PHP \\
\midrule
    $r_1$ & -0.09 & 0.45 & 0.36 & 0.46 & 0.74 & 1.76 & 0.18 & 1.05 & 0.43 & 0.62 & 0.8 & 1.62 & 0.49 & 0.61 & 0.38 & 0.56 & 0.39 & 0.77 \\
\midrule
         $r_{2,1}$ & 0.53 & 0.44 & 0.47 & 0.47 & 0.67 & 1.06 & 0.36 & 0.71 & 0.94 & 0.62 & 0.69 & 1.02 & 0.66 & 0.65 & 0.55 & 0.5 & 0.38 & 0.92 \\
\cdashline{1-20}
         $r_{2,5}$ & 0.2 & 0.02 & 0.21 & 0.3 & 0.27 & 0.24 & 0.24 & 0.65 & 0.57 & 0.41 & 0.51 & 0.36 & 0.37 & 0.33 & 0.31 & 0.17 & 0.18 & 0.35 \\
\cdashline{1-20}
         $r_{2,10}$ & 0.63 & 0.12 & 0.42 & 0.44 & 0.33 & -0.06 & 0.3 & 0.61 & 0.65 & 0.41 & 0.5 & 0.22 & 0.41 & 0.29 & 0.33 & 0.16 & 0.19 & 0.48 \\

\bottomrule
\end{tabular}
}

\end{minipage}
\end{tabular}
}
\captionsetup{type=table}
\vspace{-0.5em}  
\caption{
    Reported values for $r_1$ and $r_{2,k}$ for $k \in {1, 5, 10}$
    % calculated by Equation~\ref{eq:r1_r2} and Equation~\ref{eq:r1_r2}
    for CodeT5, CodeBERT, and UniXCoder for code summarization across 6 languages.
}\label{table:r1_r2}
\end{center}
\vspace{-1em}
\end{table*}


==> tables/seq_prob.tex <==
\begin{table*} [t]
\begin{center}
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{p{12cm}p{7cm}}
\begin{minipage}{0.75\textwidth}
\resizebox{\textwidth}{!}{
\begin{tabular}{lc c c lc c c c c cc}
\toprule
Models & Stages & Ruby & JavaScript & Go & Python & Java & PHP & Concode \\
\midrule
    CodeT5 & $P_{\theta_{fine-tuned}}(y=\hat{y_i} \mid x_i)$ & 1.45\% & 1.63\% & 3.22\% & 2.41\% & 4.02\% & 3.45\% & 33.56\% \\
       % & $P_{\theta_{improved}}(y=\hat{y_i} \mid x_i)$       & 7.10\% & 21.06\% & 19.82\% & 20.97\% & 17.13\% & 24.70\% & 41.25\% \\
       & $P_{\theta_{improved}}(y=\hat{y_i} \mid x_i)$       &\textbf{7.10\%} & \textbf{21.06\%} & \textbf{19.82\%} & \textbf{20.97\%} & \textbf{17.13\%} & \textbf{24.70\%} & \textbf{41.25\%} \\
       %&          & Our (multi-languages) & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
% \cdashline{2-10}
%        & $PPL$    & Baseline          & 1.44 & 1.40 & 1.41 & 1.32 & 1.35 & 1.22 & 1.26 \\
%        &          & Our (specific language) & \textbf{1.59} & \textbf{1.63} & \textbf{1.65} & \textbf{1.50} & \textbf{1.47} & \textbf{1.31} & \textbf{1.31} \\
%        %&          & Our (multi-languages) & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
\midrule
    CodeBERT & $P_{\theta_{fine-tuned}}(y=\hat{y_i} \mid x_i)$ & 0.33\% &  & 1.59\% & 1.61\% & 1.90\% & 3.52\% & - \\
       & $P_{\theta_{improved}}(y=\hat{y_i} \mid x_i)$ &  \textbf{1.52\%} & \textbf{7.73\%} & \textbf{10.65\%} & \textbf{13.90\%} & \textbf{7.86\%} & \textbf{14.26\%} & - \\
% \cdashline{2-10}
%          & $PPL$    & Baseline          & 78.11 & 368.89 & 15.97 & 22.97 & 24.24 & 16.96 & - \\
%          &          & Our      & \textbf{101.99} & \textbf{399.70} & \textbf{30.60} & \textbf{52.88} & \textbf{34.87} & \textbf{26.38} & - \\
\bottomrule
\end{tabular}
}

\end{minipage}
\end{tabular}
}
\captionsetup{type=table}
\vspace{-0.5em}  
\caption{
    Averaged probability of the greedy decoding generated sequences by $\theta_{fine-tuned}$ and $\theta_{improved}$ on test data for code summarization (CodeT5, CodeBERT) and code generation (CodeT5). The higher probability for each model is in bold.
}\label{table:seq_prob}
\end{center}
\vspace{-1em}
\end{table*}


==> tables/stats.tex <==
\begin{table} [t]
\captionsetup{}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lc c c c c c}
\toprule
Beam sizes & $r$ & $R^2$ & least square equation \\ 
\midrule
1 & 0.77 & 0.592 & $y=0.362x+0.414$ \\
\midrule
5 & 0.27 &  0.072 & $y=0.090x+0.258$ & \\
\midrule
10 & -0.43 & 0.185 & $y=-0.177x+0.471$ & \\
\bottomrule
\end{tabular}
}

\vspace{-0.5em}  
\caption{
    Descriptive statistics for ($r_1$, $r_{2,k})$ for $k \in {1, 5, 10}$. $r$ represents pearson correlation, and $R^2$ represents coefficient of determination in linear regression.
    }\label{table:stats}
\vspace{-1em}
\end{table}

